Recommending Metamodel Concepts during Modeling Activities with Pre-Trained Language Models

The design of conceptually sound metamodels that embody proper semantics in relation to the application domain is particularly tedious in Model-Driven Engineering. As metamodels define complex relationships between domain concepts, it is crucial for a modeler to define these concepts thoroughly while being consistent with respect to the application domain. We propose an approach to assist a modeler in the design of a metamodel by recommending relevant domain concepts in several modeling scenarios. Our approach does not require to extract knowledge from the domain or to hand-design completion rules. Instead, we design a fully data-driven approach using a deep learning model that is able to abstract domain concepts by learning from both structural and lexical metamodel properties in a corpus of thousands of independent metamodels. We evaluate our approach on a test set containing 166 metamodels, unseen during the model training, with more than 5000 test samples. Our preliminary results show that the trained model is able to provide accurate top-$5$ lists of relevant recommendations for concept renaming scenarios. Although promising, the results are less compelling for the scenario of the iterative construction of the metamodel, in part because of the conservative strategy we use to evaluate the recommendations.

==> content/algo_rq3.tex <==
\begin{algorithm}
  \caption{Metamodel Iterative Construction
    \label{alg:iterative_construction}}
  \begin{algorithmic}[1]
    \Require{$tree$ -- the metamodel tree representation}
    \State \Call{Sample\_generation}{$tree$}
    \Statex
    
    \Function{Generate\_test\_sample}{$nodes$, $mask\_node$}
      \Let{$tree\_string$}{None}
      \Let{$ground\_truth$}{None}
      \\
      \For{$n \in nodes$}
        \If{$n == mask\_node$}
            \Let{$tree\_string$}{$tree\_string + mask\_token$}
            \Let{$ground\_truth$}{$n.name$}
        \Else
            \Let{$tree\_string$}{$tree\_string + n.name$}
        \EndIf
      \EndFor
      \State \Return{$tree\_string$, $ground\_truth$}
    \EndFunction
    \\
    \Function{Sample\_generation}{$tree$}
      \Let{$selected\_nodes$}{\{\}} \Comment{set to avoid duplicates}
      \Let{$cls\_ok$}{[]}
      \Let{$test\_samples$}{[]}
      \Let{$current\_cls$}{None}
      \\
      \While{$cls\_ok.size < tree.cls.size$}
        \If{$current\_cls \notin cls\_ok$}
            \State $cls\_ok.add(current\_cls)$
        \EndIf
        \If{$current\_cls ==$ None}
          \State {\color{blue} // \textit{get next classifier and generate sample} }
          \Let{$current\_cls$}\Call{find\_next\_cls}{}
          \State $selected\_nodes.add(current\_cls)$
          \State $test\_samples.add($\Call{Generate\_test\_sample}{
            \Statex[4] $selected\_nodes$, $current\_cls$}
            \Statex[3] $)$
          \EndIf
            
            \For{$attr \in current\_cls.attributes$}
            \State {\color{blue} // \textit{attributes sample of current classifier} }
                \State $selected\_nodes.add(attr)$
                \State $test\_samples.add($\Call{Generate\_test\_sample}{
                    \Statex[4] $selected\_nodes$, $attr$}
                    \Statex[3] $)$
            \EndFor
            \For{$assoc \in current\_cls.associations$}
                \State {\color{blue} // \textit{get classifier linked by the association} }
                \Let{$linked\_cls$}{\Call{resolve\_cls}{assoc}}
                \State $selected\_nodes.add(linked\_cls)$
                \State $test\_samples.add($\Call{Generate\_test\_sample}{
                    \Statex[4] $selected\_nodes$, $linked\_cls$}
                    \Statex[3] $)$
                    
                \State {\color{blue} // \textit{then generate association test sample} }
                \State $selected\_nodes.add(assoc)$
                \State $test\_samples.add($\Call{Generate\_test\_sample}{
                    \Statex[4] $selected\_nodes$, $assoc$}
                    \Statex[3] $)$
            \EndFor
        \State {\color{blue} // \textit{the next classifier is one that is reachable through an association by the current one} }
        \Let{$current\_cls$}{\Call{find\_next\_reachable\_cls}{}}
      \EndWhile
      \State \Return{$test\_samples$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}


==> tables/test_set_distribution.tex <==
\begin{table*}[!t]
\caption{[RQ3] -- Distribution of each type of prediction in the test set according to the number of elements in the available context (\textit{i.e.,} metamodel elements that have already been designed).}
    \centering
    \small
    \renewcommand{\arraystretch}{1.2}
    \setlength{\arrayrulewidth}{.5pt}
    \begin{tabular}{c|ccc} \toprule
        context size & \# class tests & \# attribute tests & \# association tests \\ \midrule
        \textbf{[1-10]} & 577 & 452 & 590  \\
        \textbf{[11-20]} & 326 & 277 & 688  \\
        \textbf{[21-30]} & 209 & 203 & 624  \\
        \textbf{[31-40]} & 160 & 159 & 470  \\
        \textbf{[41-50]} & 87 & 92 & 296  \\
        \textbf{[51-60]} & 51 & 53 & 165  \\
        \textbf{[61-70]} & 17 & 29 & 104  \\
        \textbf{[71-80]} & 8 & 21 & 55  \\
        \textbf{[81-250]} & 25 & 39 & 291 \\
        \bottomrule
    \end{tabular}
    
    \label{tab:rq3_test_set}
\end{table*}


==> tables/test_set_global_stats.tex <==
\begin{table*}[!t]
\caption{Test set statistics. Number of test samples for each prediction task.}
    \centering
    \small
    \begin{tabular}{ccccc} \toprule
        & Metamodels & Classes & Attributes & Associations \\ \midrule
        \textbf{\# test samples} & 166 & 1626 & 1325 & 3296 \\
        \bottomrule
    \end{tabular}
    
    \label{tab:test_set}
\end{table*}
